Competitive epidemic networks with multiple survival-of-the-fittest outcomes

We use a deterministic model to study two competing viruses spreading over a two-layer network in the Susceptible--Infected--Susceptible (SIS) framework, and address a central problem of identifying the winning virus in a "survival-of-the-fittest" battle. Existing sufficient conditions ensure that the same virus always wins regardless of initial states. For networks with an arbitrary but finite number of nodes, there exists a necessary and sufficient condition that guarantees local exponential stability of the two equilibria corresponding to each virus winning the battle, meaning that either of the viruses can win, depending on the initial states. However, establishing existence and finding examples of networks with more than three nodes that satisfy such a condition has remained unaddressed. In this paper, we prove that, for any arbitrary number of nodes, such networks exist. We do this by proving that given almost any network layer of one virus, there exists a network layer for the other virus such that the resulting two-layer network satisfies the aforementioned condition. To operationalize our findings, a four-step procedure is developed to reliably and consistently design one of the network layers, when given the other layer. Conclusions from numerical case studies, including a real-world mobility network that captures the commuting patterns for people between $107$ provinces in Italy, extend on the theoretical result and its consequences.

==> Figures/figure_explanations.tex <==
different_initconds_2
In this figure we show the consequences of different initial conditions in a doubly stable system. The parameters used are those for the original example system. The initial conditions, represented as $(x_1, x_2, y_1, y_2)$, are $(0.1, 0.1, 0.05, 0.05)$ and $(0.09, 0.09, 0.06, 0.06)$.

different_initconds_virusXwins
This pair of figures are the time series plots corresponding to the phase space plots in different_initconds_2. Each figure represents one of the trajectories, ending up in one of the two boundary equilibria.

different_turnoverrates
In this figure we see what a change to the turnover rate can do to a system. The turnover rate is a scaling parameter applied simultaneously to the D and the B matrices, which does not change the stability properties of the equilibria but does change the regions of attraction in a doubly stable system. The parameters used are those for the original example system first, then virus 2 is sped up with a factor of 1.2.

winner_graph
This map depicts a section of the state space where initial states have been placed in a dense grid. The parameters used are those for the original example system. The section is intended to represent a number of plausible initial scenarios where neither virus infects a large portion of the population yet. This becomes a representation of the regions of attraction.

winner_graph_virus1faster
This map is generated using the same principles as for winner_map, only here the turnover rate of virus 1 is increased by a factor of 1.2. As a consequence we can see a clear change to the regions of attraction.
